Stable and Scalable Bundle Adjustment of Holistic 3D Structures

Bundle Adjustment (BA) is a cornerstone of 3D computer vision and has benefited from decades of advances in sparse optimization and numerical methods. It was originally developed for jointly optimizing camera intrinsics, poses and sparse 3D points. While extensions incorporate lines and other primitives, integrating richer geometric structures such as parallelism, coplanarity, or wireframes often introduces significantly increased computational cost and reduced numerical stability. In this paper, we propose a unified framework that extends bundle adjustment to jointly optimize geometric features and higher-order relations. We first introduce a taxonomy that distinguishes scalable geometric features with direct 2D measurements (e.g., points and lines), from groups encoding higher-order relations (e.g., coplanarity, parallelism, etc.), where we show that groups can be modeled as camera-like entities within the bundle adjustment framework. Building on this formulation, we propose that both group constraints and cross-feature relations (i.e., point-line associations) can be expressed through 2D reprojection measurements. By formulating group-induced and cross-feature reprojection errors, we preserve the sparsity structure of classical point-based BA under Schur elimination, while avoiding direct 3D regularization that degrades the conditioning and stability. Experiments on both real-world and synthetic datasets demonstrate runtime performance comparable to classical point-only bundle adjustment, while producing significantly richer 3D structures and improved geometric accuracy.

==> figs/fig_visualizations.tex <==
\begin{figure}[tb]
\centering
\def\visimg{figs/imgs/visualizations}
\newlength{\rowha}\setlength{\rowha}{30pt}
\newlength{\rowhb}\setlength{\rowhb}{57pt}
\setlength{\tabcolsep}{0.5pt}
%
% Row 1: 4 ScanNet++ (equal width) + 2 ETH3D (grouped)
\begin{tabular}{@{}cccccc@{}}
\includegraphics[width=0.15\linewidth, height=\rowha, trim={411 267 540 419}, clip]{\visimg/scannetpp_21d970d8de} &
\includegraphics[width=0.15\linewidth, height=\rowha, trim={577 312 524 413}, clip]{\visimg/scannetpp_38d58a7a31} &
\includegraphics[width=0.15\linewidth, height=\rowha, trim={540 282 668 422}, clip]{\visimg/scannetpp_7831862f02} &
\includegraphics[width=0.15\linewidth, height=\rowha, trim={537 237 480 341}, clip]{\visimg/scannetpp_f3d64c30f8} &
\includegraphics[width=0.15\linewidth, height=\rowha, trim={656 250 601 342}, clip]{\visimg/eth3d_courtyard} &
\includegraphics[width=0.22\linewidth, height=\rowha, trim={597 423 880 481}, clip]{\visimg/eth3d_delivery_area_view1} \\
\parbox{0.15\linewidth}{\centering\tiny \textit{21d970d8de} (ScanNet++)} &
\parbox{0.15\linewidth}{\centering\tiny \textit{38d58a7a31} (ScanNet++)} &
\parbox{0.15\linewidth}{\centering\tiny \textit{7831862f02} (ScanNet++)} &
\parbox{0.15\linewidth}{\centering\tiny \textit{f3d64c30f8} (ScanNet++)} &
\parbox{0.15\linewidth}{\centering\tiny \textit{Courtyard} (ETH3D)} &
\parbox{0.22\linewidth}{\centering\tiny \textit{Delivery Area} (ETH3D)} \\
\end{tabular}
\\[1pt]
% Row 2: 7Scenes + 1DSfM
\begin{tabular}{@{}ccc@{}}
\includegraphics[width=0.25\linewidth, height=\rowhb, trim={536 167 581 361}, clip]{\visimg/7scenes_fire} &
\includegraphics[width=0.45\linewidth, height=\rowhb, trim={0 0 0 338}, clip]{\visimg/T} &
\includegraphics[width=0.28\linewidth, height=\rowhb, trim={400 0 200 120}, clip]{\visimg/1dsfm_Gendarmenmarkt} \\
\parbox{0.24\linewidth}{\centering\tiny \textit{Fire} (7Scenes)} &
\parbox{0.43\linewidth}{\centering\tiny \textit{Tower of London} (1DSfM)} &
\parbox{0.31\linewidth}{\centering\tiny \textit{Gendarmenmarkt} (1DSfM)} \\
\end{tabular}
%
\caption{\textbf{Visualizations of bundle adjusted holistic 3D structures.}}
\label{fig::visualizations}
\end{figure}


==> figs/fig_visualizations_v2.tex <==
\begin{figure}[tb]
\centering
\def\visimg{figs/imgs/visualizations}
\newlength{\visrowh}\setlength{\visrowh}{38pt}
\setlength{\tabcolsep}{4pt}
%
\begin{tabular}{@{}ccc@{}}
\includegraphics[width=0.25\linewidth, height=\visrowh, trim={440 232 668 422}, clip]{\visimg/scannetpp_7831862f02} &
\includegraphics[width=0.27\linewidth, height=\visrowh, trim={506 250 551 382}, clip]{\visimg/eth3d_courtyard} &
\includegraphics[width=0.25\linewidth, height=\visrowh, trim={260 160 240 180}, clip]{\visimg/1dsfm_Tower_of_London_aligned} \\
\parbox{0.27\linewidth}{\centering\tiny \textit{7831862f02} (ScanNet++)} &
\parbox{0.27\linewidth}{\centering\tiny \textit{Courtyard} (ETH3D)} &
\parbox{0.27\linewidth}{\centering\tiny \textit{Tower of London} (1DSfM)} \\[3pt]
%
\includegraphics[width=0.25\linewidth, height=\visrowh, trim={537 197 580 321}, clip]{\visimg/scannetpp_f3d64c30f8} &
\includegraphics[width=0.27\linewidth, height=\visrowh, trim={597 423 880 481}, clip]{\visimg/eth3d_delivery_area_view1} &
\includegraphics[width=0.27\linewidth, height=\visrowh, trim={550 190 450 210}, clip]{\visimg/1dsfm_Gendarmenmarkt_aligned} \\
\parbox{0.27\linewidth}{\centering\tiny \textit{f3d64c30f8} (ScanNet++)} &
\parbox{0.27\linewidth}{\centering\tiny \textit{Delivery Area} (ETH3D)} &
\parbox{0.27\linewidth}{\centering\tiny \textit{Gendarmenmarkt} (1DSfM)} \\
\end{tabular}
%
\caption{\textbf{Visualizations of bundle adjusted holistic 3D structures.} Parallel lines are colored the same. Note that lines and planes are optimized as infinite entities in the bundle adjustment, and their extents in the figures are only for illustration purpose.}
\label{fig::visualizations}
\end{figure}


==> tabs/sfm_results.tex <==
\begin{table}[tb]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\caption{\textbf{Evaluating the effectiveness of bundle adjustment in full structure-from-motion pipelines}. Camera pose accuracy is measured by relative pose AUCs.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l cccc cccc}
\toprule
& \multicolumn{4}{c}{Hypersim~\cite{roberts:2021} (8 scenes)} & \multicolumn{4}{c}{ScanNet++~\cite{yeshwanth2023scannet++} (20 scenes)} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& AUC@1\textdegree & AUC@3\textdegree & AUC@5\textdegree & AUC@10\textdegree & AUC@1\textdegree & AUC@3\textdegree & AUC@5\textdegree & AUC@10\textdegree \\
\midrule
COLMAP & 83.6 & 89.3 & 90.4 & 92.2 & 66.1 & 84.0 & 86.0 & 87.5 \\
Point-Line SfM & 88.3 & 92.2 & 93.2 & 94.0 & 67.0 & 84.7 & 86.7 & 89.2 \\
Holistic SfM (Ours) & \textbf{88.6} & \textbf{92.5} & \textbf{93.4} & \textbf{94.2} & \textbf{69.4} & \textbf{87.4} & \textbf{89.4} & \textbf{90.6} \\
\midrule
& \multicolumn{4}{c}{ETH3D~\cite{schops2017multi} (11 scenes)} & \multicolumn{4}{c}{7Scenes~\cite{7scenes} (7 scenes)} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& AUC@1\textdegree & AUC@3\textdegree & AUC@5\textdegree & AUC@10\textdegree & AUC@1\textdegree & AUC@3\textdegree & AUC@5\textdegree & AUC@10\textdegree \\
\midrule
COLMAP & \textbf{12.9} & 50.2 & 66.4 & 77.6 & \textbf{1.3} & 22.9 & 48.7 & 75.5 \\
Point-Line SfM & 12.2 & 49.4 & 67.1 & 79.6 & 1.2 & 23.1 & 48.9 & 76.8 \\
Holistic SfM (Ours) & 12.5 & \textbf{50.4} & \textbf{68.1} & \textbf{80.4} & \textbf{1.3} & \textbf{24.3} & \textbf{50.8} & \textbf{78.4} \\
\bottomrule
\end{tabular}%
}
\label{tab:sfm_results}
\end{table}


==> tex/related_work_v0.tex <==
\noindent
\textbf{Advances in Bundle Adjustment.}
Bundle adjustment \cite{triggs2000bundle} has been widely studied and applied in 3D reconstruction for decades. Sparse matrix techniques and the Schur complement trick \cite{hartley2003multiple} have enabled efficient solutions by exploiting the bipartite structure between cameras and 3D points. 
There have been many efforts to improve its scalability via parallel/distributed computing \cite{agarwal2010bundle,wu2011multicore,fan2025daba} and advanced solvers \cite{lourakis2009sba,jeong2011pushing}. Other advances also include robust cost functions \cite{zach2014robust}, incremental formulation \cite{kaess2011isam2}, and differentiable BA for end-to-end learning \cite{tang2018ba,teed2021droid}. Building upon these advances, several open-sourced libraries have emerged and become standard tools, notably including g2o \cite{kummerle2011g}, Ceres solver \cite{ceres-solver}, GTSAM \cite{dellaert2012factor}, etc. These libraries work together with sparse linear algebra libraries \cite{chen2008algorithm, davis2019algorithm} and provide a nice ecosystem for modern developments of geometric 3D vision, enabling multiple reliable systems on structure-from-motion \cite{snavely2006photo,wu2011visualsfm,schonberger2016structure,moulon2016openmvg} and SLAM \cite{klein2007parallel,engel2014lsd,mur2015orb} across years. Recently, bundle adjustment is also proved to be effective in refining the poses and geometry of feedforward 3D models \cite{wang2024vggsfm,wang2025vggt,wang2025pi}. In this work, we introduce a new unified framework extending bundle adjustment to handle holistic 3D structures with higher-level primitives and relations.

~\\
\noindent
\textbf{Geometric Primitives in Optimization.}
While bundle adjustment is widely considered to work with points, generalizing it to geometric primitives dates back to as early as 30 years ago \cite{hartley1996object}. However, most recent works tackling primitives \cite{nicholson2018quadricslam,yang2019cubeslam,liao2020object,laidlow2022simultaneous,wu2023object} directly optimize high-dimensional variables rather than considering their relations to its associated features, preventing them to combine with the classical bundle adjustment with 3D points. There are relatively more studies on the optimization of 3D lines and planes. In \cite{bartoli2004framework}, Bartoli and Sturm formalizes bundle adjustment on top of infinite 3D lines with orthonormal parameterization of Plucker coordinates, which are employed in many modern line-based optimization systems \cite{zuo2017robust,Liu_2023_LIMAP,liu2024robust,xu2025airslam}. Some of these line-based systems also benefit from vanishing points \cite{rother2002new,toldo2008robust}, Manhattan assumptions \cite{coughlan2000manhattan} and its variants \cite{schindler2004atlanta,li2023hong}, and deep monocular priors \cite{tan2025planarsplatting,ke2026interacted}. 
Going one step further, planes are omnipresent in manmade environments. The modeling of planar constraints in optimization can date back to several decades ago, including modeling two-view homography \cite{faugeras1988motion}, auto calibrations \cite{triggs1998autocalibration}, and explicit re-parameterization of 3D structures \cite{bartoli2003constrained}. The idea of incorporating two-view homography constraints is recently also revisited in \cite{zhou2023efficient}, yet this formulation iterates over image pairs and cannot benefit from long feature tracks. While explicit re-parameterization of 3D structures conceptually makes sense, the feature-plane associations in practice are oftentimes noisy which cannot be robustly modeled with explicit parameterization. Many recent works model 3D point-plane associations with a soft regularization term \cite{taguchi2013point,li2020leveraging,chen2023monocular,shu2023structure}, and they are also extended to lines \cite{li2020leveraging,bai2024consistent}. However, contrary to point-to-plane 3D distance in the context of LiDAR/RGBD-SLAM \cite{ma2016cpa,geneva2018lips,zhou2020fast,chen2022vip} which is able to benefit from a principled noise model on 3D points, these monocular sytems all use 3D errors on its absolute scale with some heuristic-based weighting. Our general proposed framework is able to optimize many different types of primitives, with an unified residual formulation in pixel space that implicitly model the noise of each associations. 

~\\
\textbf{Modeling of Point-Line Associations.}
Wireframes are omnipresent in man-made environments. The advent of deep neural networks makes it possible to perform 2D wireframe prediction from single images \cite{zhou2019learning,xue2020holistically}. The wireframe representation has also benefited feature matching, with either junction-aware heuristics \cite{ma2019line,xu2025airslam} or machine learning \cite{pautrat2023gluestick}. 
While recent line-based reconstruction systems \cite{Liu_2023_LIMAP,liu2024robust} model point-line associations in optimization via 3D point-to-line distance regularization, they face computational challenges as the dense coupling between shared junctions disrupts the sparse structure, requiring expensive Schur complement operations especially with dense solvers. Our method overcomes this bottleneck through a reformulation that preserves sparsity while fully exploiting wireframe constraints.

